An Implementation Model for Interaction Nets

To study implementations and optimisations of interaction net systems we propose a calculus to allow us to reason about nets, a concrete data-structure that is in close correspondence with the calculus, and a low-level language to create and manipulate this data structure. These work together so that we can describe the compilation process for interaction nets, reason about the behaviours of the implementation, and study the efficiency and properties.

==> eptcsdata.tex <==
\providecommand{\firstpage}{66}
\providecommand{\publicationstatus}{A. Middeldorp and F. van Raamsdonk (Eds.): 8th International\\ Workshop on Computing with Terms and Graphs (TERMGRAPH 2014)\\
EPTCS 183, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.183.5}{10.4204/EPTCS.183.5}}

